Uncertainty in Extreme Multi-label Classification

Uncertainty quantification is one of the most crucial tasks to obtain trustworthy and reliable machine learning models for decision making. However, most research in this domain has only focused on problems with small label spaces and ignored eXtreme Multi-label Classification (XMC), which is an essential task in the era of big data for web-scale machine learning applications. Moreover, enormous label spaces could also lead to noisy retrieval results and intractable computational challenges for uncertainty quantification. In this paper, we aim to investigate general uncertainty quantification approaches for tree-based XMC models with a probabilistic ensemble-based framework. In particular, we analyze label-level and instance-level uncertainty in XMC, and propose a general approximation framework based on beam search to efficiently estimate the uncertainty with a theoretical guarantee under long-tail XMC predictions. Empirical studies on six large-scale real-world datasets show that our framework not only outperforms single models in predictive performance, but also can serve as strong uncertainty-based baselines for label misclassification and out-of-distribution detection, with significant speedup. Besides, our framework can further yield better state-of-the-art results based on deep XMC models with uncertainty quantification.

==> tables/alldeepacc.tex <==
\begin{table}[!h]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc}
\cline{2-10}
    & P@1 & P@3 & P@5 & P@1 & P@3 & P@5 & P@1 & P@3 & P@5 \\ \hline 
 Method & \multicolumn{3}{c|}{\eurlex} & \multicolumn{3}{c|}{\wikis}  & \multicolumn{3}{c}{\amzsmall}\\ \hline
    AnnexML~\cite{tagami2017annexml} &  79.66 &  64.94 &  53.52 &  86.46 &  74.28 &  64.20 & 42.09 &  36.61 &  32.75 \\
    DiSMEC~\cite{babbar2017dismec} &  83.21 &  70.39 &  58.73 &  84.13 &  74.72 & 65.94 & 44.78 &  39.72 &  36.17\\
    PfastreXML~\cite{jain2016extreme} &  73.14 &  60.16 &  50.54 &  83.57 &  68.61 &  59.10 & 36.84 &  34.23 &  32.09 \\
    Parabel~\cite{prabhu2018parabel} &  82.12 &  68.91 &  57.89 &  84.19 &  72.46 &  63.37 & 44.91 &  39.77 &  35.98 \\
    eXtremeText~\cite{wydmuch2018no} &  79.17 &  66.80 &  56.09 &  83.66 &  73.28 &  64.51 & 42.54 &  37.93 &  34.63 \\
    Bonsai~\cite{khandagale2020bonsai} &  82.30 &  69.55 &  58.35 &  84.52 &  73.76 &  64.69 & 45.58 &  40.39 &  36.60 \\
    XML-CNN~\cite{liu2017deep} &  75.32 &  60.14 &  49.21 &  81.41 &  66.23 &  56.11 & 33.41 &  30.00 &  27.42 \\
 %   XR-Linear~\cite{yu2020pecos} &  84.14 &  72.05 &  60.67 &  85.75 &  75.79 &  66.69 & 43.38 &  38.40 &  34.77 \\
    AttentionXML~\cite{you2019attentionxml} &  85.49 &  73.08 &  61.10 &  87.05 &  77.78 &  68.78 & 45.66 &  40.67 &  36.94 \\
    X-Transformer~\cite{chang2020xmctransformer} &  85.82 &  73.23 & 61.18 &  87.79 &  78.43 &  69.74  &46.45 & 40.82 & 36.71\\ 
    LightXML~\cite{jiang2021lightxml} &  85.60 & 74.10 & 62.00 & 87.84 & 77.26 &67.99 & 47.30 &  42.20 &  38.50 \\
    \xrtransformer~\cite{zhang2021fast} & 87.17 & 74.51 &  61.51 &  87.89 & 78.69 &  69.08 & 49.00 & 43.68 & 39.81\\ \hline
    \xrtransformer with \emph{Boosted Bagging} & \bf 88.10 & \bf  75.71 & \bf  62.21 & \bf 88.54 & \bf  79.68 & \bf  70.31 & \bf 49.95 & \bf 44.58 & \bf 40.67\\ \hline
\end{tabular}
}

\caption{Predictive performance of various single XMC models and our approach using \xrtransformer as the base XMC model on \eurlex and \wikis. P@$k$ represents precision with top-$k$ predicted labels.}
 \label{table:alldeepacc}
\end{table}


==> tables/datasets.tex <==
\begin{table}[!h]
\centering
\caption{The statistics of six experimental datsets. Note that $n_{\text{train}}, n_{\text{test}}$ are the numbers of training and testing instnaces. 
        $\abs{\cD_{\text{train}}}$ and $\abs{\cD_{\text{test}}}$ refer to the number of word tokens in the training and test corpus, respectively.
        $d$ is the dimension of \tfidf feature vector.
        $L$ is the number of labels while $\bar{L}$ the average number of labels per instance.
        $\bar{n}$ the average number of instances per label.
}
\label{table:datasets}
%\resizebox{1.0\textwidth}{!}{
    \begin{tabular}{c|rrrrrrrr}
    \toprule
        Dataset            & $n_{\text{train}}$ & $n_{\text{test}}$ & $\abs{\cD_{\text{train}}}$ &  $\abs{\cD_{\text{test}}}$ & $d$       & $L$       & $\bar{L}$ & $\bar{n}$ \\
        \midrule
        \eurlex         &       15,449    &           3,865  &              19,166,707  &                 4,741,799 &   186,104 &     3,956 &     5.30  &     20.79 \\
        \wikis          &       14,146    &           6,616  &              29,603,208  &                13,513,133 &   101,938 &    30,938 &    18.64  &      8.52 \\
        \amzsmall       &      490,449    &         153,025  &             119,981,978  &                36,509,660 &   135,909 &   670,091 &     5.45  &      3.99 \\
        \amzcat         &    1,186,239    &         306,782  &             250,940,894  &                64,755,034 &   203,882 &    13,330 &     5.04  &    448.57 \\
        \wikil          &    1,779,881    &         769,421  &           1,463,197,965  &               632,463,513 & 2,381,304 &   501,070 &     4.75  &     16.86 \\
        \amzlarge       &    1,717,899    &         742,507  &             174,559,559  &                75,506,184 &   337,067 & 2,812,281 &    36.04  &     22.02 \\
        \bottomrule
        \end{tabular}
%}
\end{table}


